Universal Gradient Methods for Stochastic Convex Optimization

We develop universal gradient methods for Stochastic Convex Optimization (SCO). Our algorithms automatically adapt not only to the oracle's noise but also to the H\"older smoothness of the objective function without a priori knowledge of the particular setting. The key ingredient is a novel strategy for adjusting step-size coefficients in the Stochastic Gradient Method (SGD). Unlike AdaGrad, which accumulates gradient norms, our Universal Gradient Method accumulates appropriate combinations of gradient- and iterate differences. The resulting algorithm has state-of-the-art worst-case convergence rate guarantees for the entire H\"older class including, in particular, both nonsmooth functions and those with Lipschitz continuous gradient. We also present the Universal Fast Gradient Method for SCO enjoying optimal efficiency estimates.

==> StochasticGradientMethod/TheMethod.tex <==
\subsection{The (Stochastic) Method}

\begin{algorithm}[tb]
  \caption{Universal Stochastic Gradient Method}
  \label{alg:StochasticGradientMethod}
  \UsingNamespace{StochaticGradientMethod}
  \begin{algorithmic}[1]
    \State \textbf{Initialize:}
    $x_0 \in \EffectiveDomain \psi$,
    $D > 0$,
    $H_0 \DefinedEqual 0$,
    $g_0 \SampledFrom \hat{g}(x_0)$.

    \For{$k = 0, 1, \ldots$}
      \State
      \LocalLabel{step:ComputeNewPoint}
      $
        x_{k + 1}
        =
        \argmin_{x \in \EffectiveDomain \psi} \{
          \DualPairing{g_k}{x} + \psi(x) + \frac{H_k}{2} \Norm{x - x_k}^2
        \}
      $.

      \State
      \LocalLabel{step:ComputeStochasticGradient}
      $g_{k + 1} \SampledFrom \hat{g}(x_{k + 1})$.

      \State
      \LocalLabel{step:UpdateRegularizationParameter}
      $
        H_{k + 1}
        \DefinedEqual
        H_k
        +
        \frac{
          \PositivePart{\hat{\beta}_{k + 1} - \frac{1}{2} H_k r_{k + 1}^2}
        }{
          D^2 + \frac{1}{2} r_{k + 1}^2
        }
      $,\par
      where
      $r_{k + 1} = \Norm{x_{k + 1} - x_k}$,
      $
        \hat{\beta}_{k + 1}
        =
        \DualPairing{g_{k + 1} - g_k}{x_{k + 1} - x_k}
      $.
    \EndFor
  \end{algorithmic}
\end{algorithm}

Our Universal Gradient Method for problem~\eqref{eq:MainProblem} with stochastic
gradient oracle is shown in \cref{alg:StochasticGradientMethod}.
As we can see, this method is very similar to its deterministic counterpart
(\cref{alg:GradientMethod}) with two fundamental differences to accommodate
stochastic feedback.
First, instead of the exact subgradients~$f'(x_k)$, we now use their
stochastic estimates~$g_k$.
Second, instead of the exact Bregman distance
$\BregmanDistance{f}(x_k, x_{k + 1})$, we now use
$\hat{\beta}_{k + 1} = \InnerProduct{g_{k + 1} - g_k}{x_k - x_{k + 1}}$, which
can be seen as the stochastic approximation of the \emph{symmetrized Bregman
distance}
$
  \hat{\beta}_f(x_k, x_{k + 1})
  \DefinedEqual
  \InnerProduct{f'(x_{k + 1}) - f'(x_k)}{x_{k + 1} - x_k}
$.
(Note that, for any $x, y \in \EffectiveDomain f$, we have
$\hat{\beta}_f(x, y) = \BregmanDistance{f}(x, y) + \BregmanDistance{f}(y, x)$.)

Next, we present the main result on the convergence of
\cref{alg:StochasticGradientMethod}
(see \cref{sec:ProofForStochasticGradientMethod} for the proof).

\begin{restatable}{theorem}{thConvergenceRateOfStochasticGradientMethod}
  \label{th:ConvergenceRateOfStochasticGradientMethod}
  Let \cref{alg:StochasticGradientMethod} be applied to
  problem~\eqref{eq:MainProblem} under
  \cref{%
    as:BoundedFeasibleSet,%
    as:AtLeastOneHolderConstantIsFinite,%
    as:StochasticGradientOracle%
  },
  and let $\bar{x}_k \DefinedEqual \frac{1}{k} \sum_{i = 1}^k x_i$ be the
  average iterate.
  Then, for all $k \geq 1$,
  \[
    \Expectation[F(\bar{x}_k)] - F^*
    \leq
    \inf_{\nu \in \ClosedClosedInterval{0}{1}}
    \frac{8 L_{\nu} D^{1 + \nu}}{k^{(1 + \nu) / 2}}
    +
    \frac{4 \sigma D}{\sqrt{k}}.
  \]
  Consequently, it suffices to make
  $
    \BigO\bigl(
      \inf_{\nu \in \ClosedClosedInterval{0}{1}}
      [\frac{L_{\nu}}{\epsilon}]^{2 / (1 + \nu)} D^2
      +
      \frac{\sigma^2 D^2}{\epsilon^2}
    \bigr)
  $
  oracle calls to reach $\Expectation[F(\bar{x}_k)] - F^* \leq \epsilon$
  for any~$\epsilon > 0$.
\end{restatable}
